Security and Privacy Issues in Deep Learning

To promote secure and private artificial intelligence (SPAI), we review studies on the model security and data privacy of DNNs. Model security allows system to behave as intended without being affected by malicious external influences that can compromise its integrity and efficiency. Security attacks can be divided based on when they occur: if an attack occurs during training, it is known as a poisoning attack, and if it occurs during inference (after training) it is termed an evasion attack. Poisoning attacks compromise the training process by corrupting the data with malicious examples, while evasion attacks use adversarial examples to disrupt entire classification process. Defenses proposed against such attacks include techniques to recognize and remove malicious data, train a model to be insensitive to such data, and mask the model's structure and parameters to render attacks more challenging to implement. Furthermore, the privacy of the data involved in model training is also threatened by attacks such as the model-inversion attack, or by dishonest service providers of AI applications. To maintain data privacy, several solutions that combine existing data-privacy techniques have been proposed, including differential privacy and modern cryptography techniques. In this paper, we describe the notions of some of methods, e.g., homomorphic encryption, and review their advantages and challenges when implemented in deep-learning models.

==> Bio.tex <==
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./BGP/HBae}}]
    {Ho Bae} received his B.Sc. degree in computer science from University College London, UK, in 2007, and his M.Sc. degree in information security from University College London, UK, in 2009. He was with SAP Labs Korea from 2012 to 2016. In 2021, he received Ph.D. degree in Bioinformatics from Seoul National University, South Korea. Since March 2021, he is working at Department of Cyber Security in Ewha Womans University, Seoul. His research interests include AI-based security, bioinformatics, and privacy.
\end{IEEEbiography}



\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./BGP/JHJang.jpg}}]
    {Jaehee Jang} received her B.S. degree in the Department of Electrical and Computer Engineering from Seoul National University in Seoul, Korea in 2016. Currently, she is pursuing a Ph.D. degree in the Department of Electrical and Computer Engineering at Seoul National University. Her research interests include privacy-preserving deep learning and federated learning.
\end{IEEEbiography}


\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./BGP/DHJung.jpg}}]
    {Dahuin Jung} received her B.S. degree in electrical engineering from University of Washington in Seattle, US in 2016. Currently, she is pursuing an integrated M.S./Ph.D. degree in electrical and computer engineering at Seoul National University. Her research interests include deep learning and representation learning.
\end{IEEEbiography}


\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./BGP/HMJang.jpg}}]
    {Hyemi Jang} received the B.S. degree in Electrical and Computer Engineering from Seoul National University, Seoul, Korea, in 2017. Currently, she is pursuing an integrated M.S./Ph.D. degree in electrical and computer engineering at Seoul National University. Her research interests include deep learning, security of neural networks and continual learning.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./BGP/HSHa.jpg}}]
    {Heonseok Ha} received his B.S. degree in electrical and computer engineering from Seoul National University in Seoul, Korea in 2014. Currently, he is pursuing an integrated M.S./Ph.D. degree in electrical and computer engineering at Seoul National University. His research interests include machine learning, privacy of neural networks and generative models.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./BGP/HGLee}}]
    {Hyungyu Lee} received his bachelor's degree in Electrical and Computer Engineering from Seoul Natonal University, Republic of Korea in 2019. Currently, he is pursuing an integrated M.S./Ph.D. degree in electrical and computer engineering at Seoul National University. There he is working in the lab of Data Science and Aritifical Intelligence Laboratory (DSAIL). His current interests are explainable AI and robustness of artificial neural networks.
\end{IEEEbiography}



\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./BGP/SRYoon}}]
    {Prof. Sungroh Yoon (S’99–M’06–SM’11)} received the B.S. degree in electrical engineering from Seoul National University, South Korea, in 1996, and the M.S. and Ph.D. degrees in electrical engineering from Stanford University, CA, USA, in 2002 and 2006, respectively, where he was a Visiting Scholar with the Department of Neurology and Neurological Sciences, from 2016 to 2017. He held research positions at Stanford University and Synopsys, Inc., Mountain View. From 2006 to 2007, he was with Intel Corporation, Santa Clara. He was an Assistant Professor with the School of Electrical Engineering, Korea University, from 2007 to 2012. He is currently a Professor with the Department of Electrical and Computer Engineering, Seoul National University, South Korea. His current research interests include machine learning and artificial intelligence. He was a recipient of the SNU Education Award, in 2018, the IBM Faculty Award, in 2018, the Korean Government Researcher of the Month Award, 2018, the BRIC Best Research of the Year, in 2018, the IMIA Best Paper Award, in 2017, the Microsoft Collaborative Research Grant, in 2017 and 2020, the SBS Foundation Award, in 2016, the IEEE Young IT Engineer Award, in 2013, and many other prestigious awards. Since February 2020, Prof. Yoon has been serving as the chairperson (minister-level position) of the Presidential Committee on the Fourth Industrial Revolution established by the Korean Government.
\end{IEEEbiography}
